Asymptotics for a special solution of the thirty fourth Painleve equation

In a previous paper we studied the double scaling limit of unitary random matrix ensembles of the form Z_{n,N}^{-1} |\det M|^{2\alpha} e^{-N \Tr V(M)} dM with \alpha > -1/2. The factor |\det M|^{2\alpha} induces critical eigenvalue behavior near the origin. Under the assumption that the limiting mean eigenvalue density associated with V is regular, and that the origin is a right endpoint of its support, we computed the limiting eigenvalue correlation kernel in the double scaling limit as n, N \to \infty such that n^{2/3}(n/N-1) = O(1) by using the Deift-Zhou steepest descent method for the Riemann-Hilbert problem for polynomials on the line orthogonal with respect to the weight |x|^{2\alpha} e^{-NV(x)}. Our main attention was on the construction of a local parametrix near the origin by means of the \psi-functions associated with a distinguished solution u_{\alpha} of the Painleve XXXIV equation. This solution is related to a particular solution of the Painleve II equation, which however is different from the usual Hastings-McLeod solution. In this paper we compute the asymptotic behavior of u_{\alpha}(s) as s \to \pm \infty. We conjecture that this asymptotics characterizes u_{\alpha} and we present supporting arguments based on the asymptotic analysis of a one-parameter family of solutions of the Painleve XXXIV equation which includes u_{\alpha}. We identify this family as the family of tronquee solutions of the thirty fourth Painleve equation.

==> figure1.tex <==
%%Created by jPicEdt 1.4-pre5: mixed JPIC-XML/LaTeX format
%%Tue Nov 07 19:54:52 CET 2006
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="80" y-min="10" y-max="65" auto-bounding="true">
%<multicurve fill-style= "none"
%    points= "(10,40);(10,40);(80,40);(80,40)"
%    />
%<multicurve fill-style= "none"
%    points= "(45,40);(45,40);(20,15);(20,15)"
%    />
%<multicurve fill-style= "none"
%    points= "(65,40);(65,40);(65,40);(65,40)"
%    />
%<text text-vert-align= "center-v"
%    anchor-point= "(65,42.5)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%S1
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(52.5,57.5)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(35,55)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%S2
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(42.5,62.5)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(25,42.5)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%S3
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(37.5,20)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(32.5,25)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(32.5,25)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(35,25)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%S4
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(55,55)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%O1
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(20,50)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%O2
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(20,30)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%O3
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(55,25)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%O4
%</text>
%<text text-vert-align= "center-v"
%    anchor-point= "(45,10)"
%    text-hor-align= "center-h"
%    text-frame= "noframe"
%    fill-style= "none"
%    >
%RH problem for Psi
%</text>
%<multicurve arrow-global-scale-width= "10"
%    fill-style= "none"
%    arrow-global-scale-length= "20"
%    left-arrow= "head"
%    points= "(65,40);(65,40);(64,40);(64,40)"
%    />
%<multicurve fill-style= "none"
%    points= "(45,40);(45,40);(20,65);(20,65)"
%    />
%<multicurve fill-style= "none"
%    left-arrow= "head"
%    points= "(25,40);(25,40);(24,40);(24,40)"
%    />
%<multicurve fill-style= "none"
%    left-arrow= "head"
%    points= "(33,52);(33,52);(32,53);(32,53)"
%    />
%<multicurve fill-style= "none"
%    left-arrow= "head"
%    points= "(33,28);(33,28);(32,27);(32,27)"
%    />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,50)(-40,15)
\linethickness{0.3mm} \put(10,40){\line(1,0){70}}
\linethickness{0.3mm}
\multiput(20,15)(0.12,0.12){208}{\line(1,0){0.12}}
\put(65,42.5){\makebox(0,0)[cc]{$\Sigma_1$}}

\put(35,55){\makebox(0,0)[cc]{$\Sigma_2$}}

\put(25,42.5){\makebox(0,0)[cc]{$\Sigma_3$}}

\put(35,25){\makebox(0,0)[cc]{$\Sigma_4$}}

\put(55,55){\makebox(0,0)[cc]{$\Omega_1$}}

\put(20,50){\makebox(0,0)[cc]{$\Omega_2$}}

\put(20,30){\makebox(0,0)[cc]{$\Omega_3$}}

\put(55,25){\makebox(0,0)[cc]{$\Omega_4$}}

\put(45,37.5){\makebox(0,0)[cc]{$0$}}

%\put(45,10){\makebox(0,0)[cc]{Figure 1: Contour for the model RH
%problem.}}

\thicklines \put(64,40){\line(1,0){1}}
\put(65,40){\vector(1,0){0.12}} \thicklines
\multiput(20,65)(0.12,-0.12){208}{\line(1,0){0.12}} \thicklines
\put(24,40){\line(1,0){1}} \put(25,40){\vector(1,0){0.12}}
\thicklines \multiput(32,53)(0.12,-0.12){8}{\line(1,0){0.12}}
\put(33,52){\vector(1,-1){0.12}} \thicklines
\multiput(32,27)(0.12,0.12){8}{\line(1,0){0.12}}
\put(33,28){\vector(1,1){0.12}}

%\linethickness{0.3mm}
%\multiput(42.14,42.18)(0.12,0.11){3}{\line(1,0){0.12}}
%\multiput(41.83,41.81)(0.1,0.12){3}{\line(0,1){0.12}}
%\multiput(41.58,41.4)(0.12,0.21){2}{\line(0,1){0.21}}
%\multiput(41.4,40.95)(0.09,0.22){2}{\line(0,1){0.22}}
%\multiput(41.29,40.48)(0.11,0.47){1}{\line(0,1){0.47}}
%\multiput(41.25,40)(0.04,0.48){1}{\line(0,1){0.48}}
%\multiput(41.25,40)(0.04,-0.48){1}{\line(0,-1){0.48}}
%\multiput(41.29,39.52)(0.11,-0.47){1}{\line(0,-1){0.47}}
%\multiput(41.4,39.05)(0.09,-0.22){2}{\line(0,-1){0.22}}
%\multiput(41.58,38.6)(0.12,-0.21){2}{\line(0,-1){0.21}}
%\multiput(41.83,38.19)(0.1,-0.12){3}{\line(0,-1){0.12}}
%\multiput(42.14,37.82)(0.12,-0.11){3}{\line(1,0){0.12}}

%\put(36.75,42.5){\makebox(0,0)[cc]{$\pi / 3$}}

%\put(36.75,37.5){\makebox(0,0)[cc]{$\pi / 3$}}

%%%%%%%%%%%%%%%%%%%smallarc4
\linethickness{0.3mm}
\multiput(48.06,40.5)(0.06,-0.5){1}{\line(0,-1){0.5}}
\multiput(47.93,40.99)(0.13,-0.49){1}{\line(0,-1){0.49}}
\multiput(47.73,41.46)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(47.46,41.89)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(47.13,42.27)(0.11,-0.13){3}{\line(0,-1){0.13}}
\multiput(46.74,42.6)(0.13,-0.11){3}{\line(1,0){0.13}}
\multiput(46.31,42.88)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(45.85,43.08)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(45.36,43.22)(0.49,-0.14){1}{\line(1,0){0.49}}
\multiput(44.86,43.28)(0.5,-0.06){1}{\line(1,0){0.5}}
\multiput(44.35,43.27)(0.51,0.01){1}{\line(1,0){0.51}}
\multiput(43.85,43.18)(0.5,0.09){1}{\line(1,0){0.5}}
\multiput(43.37,43.02)(0.48,0.16){1}{\line(1,0){0.48}}
\multiput(42.91,42.79)(0.23,0.11){2}{\line(1,0){0.23}}
\multiput(42.5,42.5)(0.21,0.15){2}{\line(1,0){0.21}}

\put(47.75,45.5){\makebox(0,0)[cc]{$2\pi / 3$}}
\end{picture}

